Spotting political social bots in Twitter: A use case of the 2019 Spanish general election

While social media has been proved as an exceptionally useful tool to interact with other people and massively and quickly spread helpful information, its great potential has been ill-intentionally leveraged as well to distort political elections and manipulate constituents. In the paper at hand, we analyzed the presence and behavior of social bots on Twitter in the context of the November 2019 Spanish general election. Throughout our study, we classified involved users as social bots or humans, and examined their interactions from a quantitative (i.e., amount of traffic generated and existing relations) and qualitative (i.e., user's political affinity and sentiment towards the most important parties) perspectives. Results demonstrated that a non-negligible amount of those bots actively participated in the election, supporting each of the five principal political parties.

==> formulae.tex <==
\section*{Mattia: formulae}

\subsection*{Analysis control flow}

\subsubsection*{Data collection}
Data have been collected from Twitter API using the SFM (https://gwu-libraries.github.io/sfm-ui/).

Tweets' \change{features}{properties} are the ones provided by the \texttt{tweet-object} data format (https://developer.twitter.com/en/docs/tweets/data-dictionary/overview/tweet-object).

We split these \addtxt{Twitter's }data in three MongoDB collections:
\begin{itemize}
    \item \textbf{tweets} ($\textbf{t}\in\mathbb{T}$), where $\textbf{t}$ is defined as a set of the following parameters: tweet id, timestamp, favorite count, retweet count, reply/retweet/quote tweet id, user id, user description, user statuses/favourite/followers/friends count, user name, user screen name, user verified status; The users properties are the ones collected at the time of the tweet's publication.
    \item \textbf{users} ($\textbf{u}\in\mathbb{U}$), where $\textbf{u}$ is defined as a set of the following parameters: user id.
\end{itemize}

\paragraph{Users}

%From now on, the users will be denoted with $\textbf{u}\in\mathbb{U}$, in case of multiple users: $\textbf{u}_1,...\textbf{u}_n$. Tweets will be $\textbf{t}\in\mathbb{T}$, in case of multiple ones: $\textbf{t}_1,...\textbf{t}_m$. 
%Both $\textbf{u}$ and $\textbf{t}$ are vectors of named features. To access them, use the upper notation, i.e., the feature "user\_id" of a tweet should be referenced as $\textbf{t}^{\text{uid}}$. For example, the user id of the $i^{th}$ tweet should be: $\textbf{t}^{\text{uid}}_i$.

%Do \textbf{not} reserve $n$ or $m$ to indicate $|\mathbb{U}|$ and $|\mathbb{T}|$.

At this point we calculated the botscore for each user. Botometer response schema is available at (\url{https://botometer.iuni.iu.edu/#!/faq#which-score}). We selected the universal score (not CAP universal!!) to be precise \texttt{response/scores/universal} which we will denoted with %$b(\textbf{u})\in[0,1]$ or 
$b_{\textbf{u}}\in[0,1]$ %according to the specific formula needs.

Given the botscore distribution, we will define the 75\textsuperscript{th} ($p_{75}\in[0,1]$) and the 95\textsuperscript{th} ($p_{95}\in[0,1]$) percentiles, respectively.

We define as \texttt{human} $\textbf{h}\in\mathbb{H}\subseteq\mathbb{U}$ those users $\textbf{u}$ with $b_{\textbf{u}}<p_{75}$ and \texttt{bots} $\textbf{b}\in\mathbb{B}\subseteq\mathbb{U}$ those users $\textbf{u}$ with $b_{\textbf{u}}>p_{95}$. We discard the users in between.

For each \texttt{bot} $\textbf{b}$, the full list of friends/followers is retrieved from Twitter APIs and stored in the users collection $\mathbb{U}$. (Formulate mathematically friends and followers??? for Gephi explanation later!)

\paragraph{Tweets}
Each tweet $\textbf{t}$ contains the following information:

\begin{align*}
    \textbf{t}=(\textbf{t}^\text{id},
                \textbf{t}^\text{type} \in \Pi,
                \textbf{t}^\text{timestamp},\\
                \textbf{t}^\text{favs} \in \mathbb{Z},
                \textbf{t}^\text{rts} \in \mathbb{Z},
                \textbf{t}^\text{uid'}\,
                \textbf{t}^\text{uid} \in \mathbb{U},
                ...)
\end{align*}
\begin{align*}
where \ \Pi = \{\texttt{quote},\texttt{retweet},\texttt{reply},\texttt{original}\},\\
\texttt{2019-10-04}<=\textbf{t}^\text{timestamp}<=\texttt{2019-11-11}\\
\end{align*}

A tweet $\textbf{t}$ is augmented with its sentiment score ($\textbf{t}^\text{sent}$) and a boolean vector of 10 elements ($\textbf{t}^\text{bags}$) .

On the one hand, the text of each tweet $\textbf{t}^{\text{text}}$ is processed to extract the sentiment score, $\textbf{t}^\text{sent}\in[0,1]$, where 0 means the most negative sentiment and 1 means the most positive sentiment, being 0.5 neutral content. ({\color{red} include the propagation of sentiment in \texttt{retweets}})

On the other hand, we define ten \textit{bag-of-words} which group keywords around certain topics. In fact, we define five \textit{bag-of-words} for political parties and five \textit{bag-of-words} for generic themes. Then, $\textbf{t}^\text{bags}$ contains \texttt{True} in those \textit{bag-of-words} in which at least one inner keyword match in $\textbf{t}^{\text{text}}$, and \texttt{False} otherwise. Each political-party oriented \textit{bag-of-word} $\mathbb{W}^p$, where $p\in\mathbb{P}$ and $\mathbb{P}$=\{\texttt{VOX}, \texttt{PP}, \texttt{Cs}, \texttt{PSOE}, \texttt{UP}\}, includes a) the selected hashtags belonging to $p$, b) real name of the leader of $p$, and c) screen names of verified users in our collection belonging to $p$. Each thematic-based \textit{bag-of-word} $\mathbb{W}^{\gamma}$, where $\gamma\in\Gamma$ and $\Gamma= \{\texttt{\text{Elecciones}}, \texttt{\text{Exhumacion}}, \texttt{\text{Catalu\~na}}, \texttt{\text{Debates}}, \texttt{\text{AbascalEH}}\}$ contains the hashtags associated to $\gamma$.

We manually labelled the 200 most important (in terms of number of interactions) users that match a regex related to the political party. {\color{red}no creo que se pueda escribir con una formula. El proceso es el mismo que se coment\'o durante la reuni\'on. Se etiquetan a mano 200 usuarios para cada partido, contando los verificados}.

\paragraph{Anonymization}
At this point, we replace all the unique identifiers with randomly generated UUID (https://en.wikipedia.org/wiki/Universally\_unique\_identifier). We drop the texts and all the metadata. 

\paragraph{Political profiler}
For each user $\textbf{u}$, for each tweet type $\tau$, for each political party $\mathbb{W}^p$, we extract the average sentiment score of the resulting tweets. 
\begin{align*}
    \forall \textbf{u} \in\mathbb{B}  ~.~ \forall \tau\in\Pi  ~.~ \forall p \in \mathbb{P},\\
    s_{\textbf{u},\tau,p}=\texttt{mean} (\textbf{t}^\text{sent} \in [0,1] \ | \ & \textbf{t}^\text{uid} = \textbf{u}^\text{uid} \\
    \wedge &\textbf{t}^\text{type} = \tau \\
%    \wedge &\textbf{t}^w = \text{True} \\
    \wedge & \exists\ w\in \mathbb{W}^p ~.~ w\in \textbf{t}^{\text{text}} \\
%    \wedge &\forall w' \neq w \in \mathbb{W}^\text{P}~.~\textbf{t}^{w'} = \text{False})
    \wedge &\forall p' \neq p ~.~ \forall w' \in \mathbb{W}^\text{p'}~.~w'\not\in \textbf{t}^{\text{text}})
\end{align*}

As before, but also including each thematic:

\begin{align*}
    \forall \textbf{u} \in\mathbb{B}  ~.~ \forall \tau\in\Pi  ~.~ \forall p \in \mathbb{P}  ~.~ \forall \gamma \in \Gamma\\
    s_{\textbf{u},\tau,p,\gamma}=\texttt{mean} (\textbf{t}^\text{sent} \in [0,1] \ | \ & \textbf{t}^\text{uid} = \textbf{u}^\text{uid} \\
    \wedge &\textbf{t}^\text{type} = \tau \\
    \wedge & \exists\ w\in \mathbb{W}^p ~.~ w\in \textbf{t}^{\text{text}} \\
    \wedge &\forall p' \neq p ~.~ \forall w' \in \mathbb{W}^\text{p'}~.~w'\not\in \textbf{t}^{\text{text}} \\
    \wedge & \exists\ q\in \mathbb{W}^\gamma ~.~ q\in \textbf{t}^{\text{text}})
\end{align*}

Each average sentiment score is a feature for the machine learning pipeline. 
For machine learning notation, we will refer to this notation: (https://nthu-datalab.github.io/ml/slides/Notation.pdf)


\begin{align*}
    \textbf{x}^\textbf{u} = &\big\{s_{\textbf{u},\tau,p} |\ \forall \tau \in \Pi~.~
    \forall p \in \mathbb{P}
    \big\} \\ 
    \cup &\big\{s_{\textbf{u},\tau,p,\gamma} |\ \forall \tau \in \Pi~.~
    \forall p \in \mathbb{P}~.~\forall \gamma \in \Gamma
    \big\} 
\end{align*}

That is to say, a feature vector $\textbf{x}$ consists of several real number in $[0,1]$, one for each bag of words $w\in\mathbb{W}$ and one for each binary combination of a political party and any other bag of words. Its label, manually assigned in the previous phase, is represented by $\textbf{y}$.

Formally, the $i^{th}$ pair example-label is indicated by $(\textbf{x}^{(i)},\textbf{y}^{(i)})$. The training set is indicated with $\mathbb{X}$.

We selected 6 classifiers $f \in \mathbb{F}$:
\begin{itemize}
    \item Random Forest ($f_1=\text{rf}(\mathbb{X})$) -- 10 tress, do not split subsets smaller than 5;
    \item Multilayer perceptron ($f_2=\text{nn}(\mathbb{X})$) -- single hidden layer, 100 nodes, ReLu activation, Adam solver with $\alpha=0.001$ and 200 training replicable interactions;
    \item SVM ($f_3=\text{svm}(\mathbb{X})$) -- $C=1.0$, $\epsilon=0.1$ with RBF kernel and 100 interaction limits with $0.001$ numerical tollerance;
    \item Naive Bayes ($f_4=\text{nb}(\mathbb{X})$) -- nothing to add;
    \item kNN ($f_5=\text{knn}(\mathbb{X})$) -- 5 neighbors, euclidean metric, uniform weight;
    \item AdaBoost (with internal Tree) ($f_6=\text{ab}(\mathbb{X})$) -- 50 estimators, SAMME.R classification algorithm and linear regression loss function.
\end{itemize}

We indicate with $\text{f}(\textbf{x'})=[\textbf{\^{y}},\text{p}(\textbf{\^{y}})]$ (where f can be any classification algorithm) the evaluation of the vector $\textbf{x'}$, the predicted labels $\textbf{\^{y}}$ and the confidence in the predicted labels $\text{p}(\textbf{\^{y}})$. If the record has an associated actual label (aka manually verified) it will be denoted with $\textbf{y'}$.

We train the classifiers with the set of manually labelled users, as described before. {\color{red}Insert F1 table for evaluation}.

We then procede to predict the political class for the users identified as bot.

For each party, all the classifiers will output a confidence score that reflects the probability of the test instance to belongs to that party. The combined probability that a user belongs to a party is given by the average of the probabilities of the users belonging to that party for each classifier. (Ensemble classifier)
Formally, for a party $p\in\mathbb{P}$ and a user $\textbf{u}$ with test vector $\textbf{x'}$:
\begin{equation}
    \text{p}(\textbf{u} \in p) = \underset{\forall f \in \mathbb{F}}{\text{mean}}\Big(f(\textbf{x'})[p]\Big) 
\end{equation}

We decided to reject the decision when the probability of the most probable class is lower than a threshold. The threshold has been set as $\delta=1-\frac{1}{|\mathbb{P}|}=0.8$. 

That is to say, the user is classified with in a party iff $\text{p}(\textbf{u} \in p) > \delta$.

If the predicted probability for a single party is lower than $\delta$, then we consider the cumulative sum of the parties with the highest probability. For example, $\text{p}(\textbf{u} \in \text{psoe})=0.5$ and $\text{p}(\textbf{u} \in \text{up})=0.45$, the cumulative sum is $0.95$. Since the sum is greater than the threshold, we accept the classification and label the users as psoe-up.

We reject the predicted class for any other user that doesn't match these conditions. 


Be aware that from the total amount of 40k bots, we only considers those that have at least one tweet with at least one party bag-of-words set to True ($\forall \textbf{b}\in\mathbb{B}~.~\exists \textbf{t}\in\mathbb{T} \ | \ \textbf{t}^\text{uid} = \textbf{b}^\text{id} \wedge \exists p \in \mathbb{P} \ | \ \textbf{t}^\text{bags}[p]=\text{True}$).

The total amount of users with at least one interaction with at least one party is 18,5k.
We use this set of users for the classification process. 
